Reliable Process for Security Policy Deployment

We focus in this paper on the problem of configuring and managing network security devices, such as Firewalls, Virtual Private Network (VPN) tunnels, and Intrusion Detection Systems (IDSs). Our proposal is the following. First, we formally specify the security requirements of a given system by using an expressive access control model. As a result, we obtain an abstract security policy, which is free of ambiguities, redundancies or unnecessary details. Second, we deploy such an abstract policy through a set of automatic compilations into the security devices of the system. This proposed deployment process not only simplifies the security administrator's job, but also guarantees a resulting configuration free of anomalies and/or inconsistencies.

==> abstract.tex <==
\fontsize{9}{11}\selectfont We focus in this paper on the problem of
configuring and managing network security devices, such as
Firewalls, Virtual Private Network (VPN) tunnels, and Intrusion
Detection Systems (IDSs). Our proposal is the following. First, we
formally specify the security requirements of a given system by
using an expressive access control model. As a result, we obtain an
abstract security policy, which is free of ambiguities, redundancies
or unnecessary details. Second, we deploy such an abstract policy
through a set of automatic compilations into the security devices of
the system. This proposed deployment process not only simplifies the
security administrator's job, but also guarantees a resulting
configuration free of anomalies
and/or inconsistencies.



==> authors.tex <==
\author{{\textmd {\textbf }}\\
  \fontsize{11}{13}\selectfont
  Stere Preda$^{\dagger}$, Nora Cuppens-Boulahia$^{\dagger}$, Fr\'ed\'eric Cuppens$^{\dagger}$,  Joaquin G. Alfaro$^{\dagger,\ddagger}$ and Laurent Toutain$^{\dagger}$\\[12pt]
  \fontsize{9}{11}\selectfont
  \textit{$^{\dagger}$GET/ENST Bretagne, 2 rue de la Ch\^ataigneraie, 35512 Cesson S\'evign\'e, France}\\
  \fontsize{9}{11}\selectfont
  \textit{\{frederic.cuppens,nora.cuppens,stere.preda,laurent.toutain\}@enst-bretagne.fr}\\[12pt]
  %
      \fontsize{9}{11}\selectfont
  \textit{$^{\ddagger}$Universitat Oberta de Catalunya, Rambla Poble Nou 156, 08018 Barcelona, Spain}\\
  \fontsize{9}{11}\selectfont
  \textit{joaquin.garcia-alfaro@acm.org}\\[12pt]
}


==> keywords.tex <==

\fontsize{9}{11}\selectfont Network Security; Security Devices;
 Security Rules; Deployment of Policies; Policy Anomalies.

